A practical approach for updating an integrity-enforced operating system

Trusted computing defines how to securely measure, store, and verify the integrity of software controlling a computer. One of the major challenges that make them hard to be applied in practice is the issue with software updates. Specifically, an operating system update causes the integrity violation because it changes the well-known initial state trusted by remote verifiers, such as integrity monitoring systems. Consequently, the integrity monitoring of remote computers becomes unreliable due to the high amount of false positives. We address this problem by adding an extra level of indirection between the operating system and software repositories. We propose a trusted software repository (TSR), a secure proxy that overcomes the shortcomings of previous approaches by sanitizing software packages. Sanitization consists of modifying unsafe installation scripts and adding digital signatures in a way software packages can be installed in the operating system without violating its integrity. TSR leverages shielded execution, i.e., Intel SGX, to achieve confidentiality and integrity guarantees of the sanitization process. TSR is transparent to package managers, and requires no changes in the software packages building and distributing processes. Our evaluation shows that running TSR inside SGX is practical; since it induces only ~1.18X performance overhead during package sanitization compared to the native execution without SGX. TSR supports 99.76% of packages available in the main and community repositories of Alpine Linux while increasing the total repository size by 3.6%.

==> Makefile <==
FILE=paper
TEXFILES=0_abstract.tex \
1_introduction.tex \
2_background.tex \
3_problems.tex \
4_design.tex \
5_implementation.tex \
6_evaluation.tex \
7_relatedwork.tex \
8_conclusion.tex \
paper.tex

pdfcmd=pdflatex -synctex=1 -interaction=nonstopmode

all: $(FILE).pdf

.PHONY: clean

clean:
	rm -f *.synctex.gz *.aux *.blg *.out  *.log *.glo *.ist *.acn $(FILE).pdf *.ist .DS_Store

$(FILE).pdf: $(FILE).tex $(TEXFILES)
	$(pdfcmd) $(FILE) ;	$(pdfcmd) $(FILE) ;	bibtex $(FILE) ; $(pdfcmd) $(FILE) ; $(pdfcmd) $(FILE)


==> discussion.tex <==
%!TEX root = paper.tex
\section{Discussion}
\label{sec:discussion}
% Pros and cons
% disclose what has, and has not, been implemented; 

\subsection{Load balancing}
\sys does not provide load balancing mechanisms. Instead, we propose to use the state-of-the-art load balancing mechanisms (\ie, nginx, apache) to cache the packages processed by \sys.

\subsection{Security}
\sys relies on the security mechanisms implemented by the upstream repositories, \ie, digitally signed packages, signed repository metafile \cite{cappos_look_2008}. In particular, if the upstream repositories get compromised, \sys will also provide access to the compromised software packages.

However, \sys addresses attacks that might be performed on it as a repository mirror, \ie, \gls{mitm}, freeze, and replay attacks \cite{cappos_look_2008}. \sys relies on the \gls{tls} to establish connection with mirrors and to expose its own repository. Furthermore, \sys mitigates freeze and replay attacks by using all mirrors defined in the policy to decide about the most up-to-date version of the package (via Byzantine quorum on all downloaded packages). Finally, \sys leverages \gls{tee} to protect itself from the privileged adversary having access to the computer where \sys is deployed. Specifically, the signing keys are securely stored inside TEE-protected memory.

\subsection{Trusted compilation}
An adversary might compromise the process of building packages. For example, she can steal signing keys, reconfiguring the \gls{cicd} process, inserting backdoors to the compiled sources. All of this allows her to build and to distribute a vulnerable version of a package. We anticipate that the security-oriented distributions will provide access to packages compiled inside TEEs which trusted compilation can be digitally proved. We expect that the policy language proposed in this paper would support the trusted compilation because such packages and their distribution would not change from the current implementation.

==> figures/highlevel.tex <==
\begin{figure}[tbp!]
\centering
% \captionsetup{skip=4pt}
\includegraphics[width=0.48\textwidth]{figures/high-level}
\caption{
    High-level overview of \sysfull (\sys). \sys is a proxy that modifies packages in a way they are safe to be installed in the integrity-enforced operating systems.
}
\label{fig:highlevel}
\end{figure}

